An Online Decision-Theoretic Pipeline for Responder Dispatch

The problem of dispatching emergency responders to service traffic accidents, fire, distress calls and crimes plagues urban areas across the globe. While such problems have been extensively looked at, most approaches are offline. Such methodologies fail to capture the dynamically changing environments under which critical emergency response occurs, and therefore, fail to be implemented in practice. Any holistic approach towards creating a pipeline for effective emergency response must also look at other challenges that it subsumes - predicting when and where incidents happen and understanding the changing environmental dynamics. We describe a system that collectively deals with all these problems in an online manner, meaning that the models get updated with streaming data sources. We highlight why such an approach is crucial to the effectiveness of emergency response, and present an algorithmic framework that can compute promising actions for a given decision-theoretic model for responder dispatch. We argue that carefully crafted heuristic measures can balance the trade-off between computational time and the quality of solutions achieved and highlight why such an approach is more scalable and tractable than traditional approaches. We also present an online mechanism for incident prediction, as well as an approach based on recurrent neural networks for learning and predicting environmental features that affect responder dispatch. We compare our methodology with prior state-of-the-art and existing dispatch strategies in the field, which show that our approach results in a reduction in response time with a drastic reduction in computational time.

==> BackgroundInfo.tex <==
% \section{Background}\label{Sec:background}
% The rest of the text in this paper builds upon the concepts of Survival Analysis, Semi-Markov Decision Processes and Monte Carlo Tree Search. We introduce each of the concepts here as part of a brief overview for benefit of the readers and make the text self-contained. We encourage readers familiar with these concepts to skip to the next section.

% \subsection{Survival Analysis}

% % Originally introduced in the field of medicine, Survival Analysis is a class of methods used to analyze data comprising of time between incidents of interest \cite{cox1984analysis}. 
% % Survival models can be parametric or non-parametric in nature, with parametric models assuming that \textit{survival time} follows a known distribution. Moreover, the risk of occurrence of events (hazard) or the time to occurrence of incidents can be chosen as the dependent variable. Specifically, we use Accelerated Failure Model (AFT) for the survival function that lets us directly model time to incidents $t$ as a function of features $w$. Formally, the survival model is
% % \[
% % f_t(t|\gamma(w)), %\, t \geq 0,
% % \]
% % where $f_t$ is a probability distribution for a continuous random 
% % variable $T$ representing the inter-arrival time, which typically depends on
% % covariates $w$ via the function $\gamma$. The model parameters can be estimated by the principled procedure of Maximum Likelihood Estimation (MLE).

% \subsection{Semi-Markov Decision Process}

% We formally model the problem of dynamic incident response as a semi-Markov decision process (SMDP) \cite{mdpHu}. An SMDP is described by a tuple $\{S,A,p_{ij}(a),t(i,j,a),\rho(i,a),\alpha \}$ where $S$ is a finite state space, $A$ is the set of actions, $p_{ij}(a)$ is the probability with which the process transitions from state $i$ to state $j$ when action $a$ is taken, $t(i,j,a)$ is a distribution over the time spent during the transition from state $i$ to state $j$ under action $a$, $\rho(i,a)$ is the reward received when action $a$ is taken in state $i$, and $\alpha$ is the discount factor for future rewards. The process is called Semi-Markovian as the transition function is not necessarily memory-less. We point out that in our case, the state space is finite but intractable and that state transition functions are unknown and difficult to model in closed form. We describe the details while formulating the problem in section \ref{Sec:SystemModel}.

% \subsection{Monte Carlo Tree Search}

% Monte Carlo Tree Search (MCTS) is a class of heuristic-based search algorithms to compute the most promising actions for a given state of a decision-making problem. Given an arbitrary state of the problem, the essential focus of the MCTS is to repeatedly simulate the system under consideration to build a search tree that keeps track of the actions taken and the rewards received. The search tree is built in a manner that balances exploration (trying new or sub-optimal actions) and exploitation (greedily exploring the best action). The simulations are then used to make a decision for the root state. 

% A related concept, introduced specifically in the context of MDP-s is sparse sampling \cite{kearns2002sparse}.

% choose the  to  procedure is Based on the Monte Carlo Method, a class of algorithms using random sampling to generate results \cite{1940s by Stanislaw Ulam}, MCTS is a heuristic search algorithm for decision processes \cite{ Bruce Abramson explored the MCTS idea in his 1987 PhD thesis}. Starting with the decision state as the root of a tree, it uses random sampling to explore the search space of actions(edges) and their resulting future states (nodes). Each time an action is explored, the tree is expanded into the future until a leaf state is found, and the rewards are back-propagated up the tree to the original action. This is repeated until the simulator runs out of time, with the actions that are expanded each time balancing exploration (trying new or less optimal actions) and exploitation (greedily exploring the best action). The action associated with the branch with the highest reward is then chosen.

% \subsection{Sparse Sampling}

% Similar to MCTS, sparse sampling performs near-optimal online MDP planning \cite{kearns2002sparse}. It accesses a generative model to randomly sample a look-ahead tree of events. But instead of considering actions based on exploration/exploitation, some subset of the available actions are considered based on their immediate (i.e. greedy) reward. Because it samples a sub space of the full MDP, the running time is dependent on the number of branches and the depth of the generated tree rather than the full state-space size. In practice, a small depth is used, and then a heuristic is used at the leaves to estimate their rewards.    

% The idea of sparse sampling can be applied to the SMDP directly, but only if the transition probabilities between the states is known. However, by construction, these probabilities are unknown and cannot be calculated in closed-form. However, such probabilities can be empirically estimated. We briefly describe a method from prior work that can learn an optimal policy by estimating such probabilities for the transformed problem $M_d$ in section \ref{Sec:OtherApproaches}.




==> HyperparamResults.tex <==
% \begin{table}
% \label{tbl:discount_factor}
% \caption{Affects of Varying Discount Factor $\gamma$} 
% \centering
% \begin{tabulary}{.9*\columnwidth}{|C|C|C|C|}

% \hline
% \textbf{Cluster} 
% & \textbf{Log-Likelihood} \\

% \hline


% \hline
% \end{tabulary}
% \vspace{-0.2in}
% \end{table}


\begin{table*}[]
\label{tbl:discount_factor}
\caption{Affects of Varying Discount Factor $\gamma$} 
\begin{tabular}{|l|l|l|l|l|}
\hline

\textbf{Gamma}                                                           & \textbf{0.8}      & \textbf{0.85}     & \textbf{0.9}     & \textbf{0.95}     \\
\hline
\hline
\begin{tabular}[l]{@{}l@{}}Avg. Response Time Change Compared to\\ Sending Closest Responder (Seconds)\end{tabular} & 0.000249 & 0.000249 & -0.0271 & 0.00887 \\
\hline
Avg. Computation Time (Seconds)                                 & 3.848    & 3.852    & 3.438   & 3.833    \\
\hline
% Avg. Response Time Change Compared to Sending Closest (\%)      &          &          &         &
% \hline
\end{tabular}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[]
\label{tbl:sim_budget}
\caption{Affects of Varying Simulation Budget $b$} 
\begin{tabular}{|l|l|l|l|}
\hline

\textbf{$b$} & \textbf{5}      & \textbf{10}     & \textbf{20}   \\
\hline
\hline
\begin{tabular}[l]{@{}l@{}}Avg. Response Time Change Compared to\\ Sending Closest Responder (Seconds)\end{tabular} & 0.0179 & -0.0271 & 0.00198  \\
\hline
Avg. Computation Time (Seconds) & 2.633    & 3.438    & 5.232   \\
\hline
% Avg. Response Time Change Compared to Sending Closest (\%)      &          &          &         &
% \hline
\end{tabular}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[]
\label{tbl:dispatch_factor}
\caption{Affects of Varying Candidate Action Factor $\epsilon$} 
\begin{tabular}{|l|l|l|l|l|}
\hline

\textbf{$\epsilon$} & \textbf{1.5}      & \textbf{2.0}     & \textbf{2.5} & \textbf{3.0}  \\
\hline
\hline
\begin{tabular}[l]{@{}l@{}}Avg. Response Time Change Compared to\\ Sending Closest Responder (Seconds)\end{tabular} & -0.0271 & -0.0271 & -0.0271  & -0.0271 \\
\hline
Avg. Computation Time (Seconds) & 0.637    & 3.438    & 12.234 & 26.861  \\
\hline
% Avg. Response Time Change Compared to Sending Closest (\%)      &          &          &         &
% \hline
\end{tabular}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[]
\label{tbl:sim_budget}
\caption{Affects of Varying Stochastic Horizon $h^{s}$} 
\begin{tabular}{|l|l|l|l|}
\hline

\textbf{$h^{s}$} & \textbf{1}      & \textbf{2}     & \textbf{3}   \\
\hline
\hline
\begin{tabular}[l]{@{}l@{}}Avg. Response Time Change Compared to\\ Sending Closest Responder (Seconds)\end{tabular} & -0.0271 & -0.0271 & -0.0271  \\
\hline
Avg. Computation Time (Seconds) & 1.305    & 3.438    & 9.251   \\
\hline
% Avg. Response Time Change Compared to Sending Closest (\%)      &          &          &         &
% \hline
\end{tabular}
\end{table*}
